Parallel local time stepping for rigid bodies represented by triangulated meshes

Discrete Element Methods (DEM), i.e.~the simulation of many rigid particles, suffer from very stiff differential equations plus multiscale challenges in space and time. The particles move smoothly through space until they interact almost instantaneously due to collisions. Dense particle packings hence require tiny time step sizes, while free particles can advance with large time steps. Admissible time step sizes can span multiple orders of magnitudes. We propose an adaptive local time stepping algorithm which identifies clusters of particles that can be updated independently, advances them optimistically and independently in time, determines collision time stamps in space-time such that we maximise the time step sizes used, and resolves the momentum exchange implicitly. It is combined with various acceleration techniques which exploit multiscale geometry representations and multiscale behaviour in time. The collision time stamp detection in space-time in combination with the implicit solve of the actual collision equations avoids that particles get locked into tiny time step sizes, the clustering yields a high concurrency level, and the acceleration techniques plus local time stepping avoid unnecessary computations. This brings a scaling, adaptive time stepping for DEM for real-world challenges into reach.

==> 33_cluster-masking.tex <==
\section{Cluster masking}
\label{section:cluster-masking}

\marginpar{This section does not add anything}

% To enable our local optimistic time step selection each particle is equipped with a "last" state ($S_{-1}$), "current" state ($S_{0}$) and "future" state ($S_{1}$).
% A "state" consists of a timestamp ($t$), the transformation ($T$) and the angular and linear momentum at that time.
% The "last" state is a true (TODO better word for this?) state and cannot be modified.
% The "current" state is correct as long as no new particles enter this cluster ($C$) before the timestamp of this state ($t_0(C)$).
% Once it is no longer possible for new particles to influence this particle before "current" state then we move "current" to "last" state.
% The "future" state is a prediction and starts as a simple linear extrapolation over the chosen time step size.
% The contact resolution step modifies the "future" state.
% Once contact resolution is complete the state is committed to the "current" state.
% 
% Particle contacts are processed in clusters that are identified in the broad phase of collision detection (see Section \ref{}).
% For each cluster we independently evaluate the time step to use.
% First we roll back the current state of each particle in the cluster to the time of the earliest current state.
% Next we use the continuous collision method previously outlined to estimate a maximum safe time step size to use per particle pair.
% From the estimated contact points, estimated time of contact and estimated relative velocity at the contact points an estimated first point of interaction can be computed.
% If accurate, stepping beyond the time of contact would result in an invalid state but not stepping as far at the first point of interaction would result in no impulse.
% A weighted average of the time of contact and first point on interaction is calculated per contact.
% The minimum of these time step sizes is taken as the time step size for the cluster.


In any given iteration of the main time step loop each cluster advances with the chosen time step as long as it retains the possibility to roll back.
A global future time stamp is give: $T_f=min_c(current_c + step_c)$.
A cluster can advance if $current_c < T_f$ (it's current time isn't greater than the time any other cluster will reach by the end of this step).

If a cluster only consists of "sleeping" particles then $step_c$ is set to the maximum allowed step size with no contact detection or resolution used.

If a cluster isn't allowed to advance in a given iteration and the same cluster is identified in the next time step then the process of selecting a time step size is skipped and the result from the last iteration is used.
This is particularly important when a large number of clusters are held from advancing by a small number of clusters with small time step sizes and therefore result in regular and expensive recomputations of the desired time step size.


==> 40_implementation.tex <==
\section{Implementation remarks}
\label{section:implementation}

\marginpar{Maybe teh Intel part goes here}
%\section{Multi threading strategy}

There are three areas which tend to dominate the run time of our simulations.
\begin{enumerate}
    \item Continuous collision detection and time step size selection within a cluster
    \item Detection of exact contact points at a given time stamp within a cluster
    \item Resolution of contacts using the sequential impulses algorithm
\end{enumerate}

The spectrum of factors that can lead to poor parallel performance make it impossible to effectively utilise parallel processes by implementing a single strategy in one place.
Instead we use multiple levels of nested task creation.
Where independent units of work exist separate tasks are spawned per item.
Where work is performed on interacting particles we colour the interaction graph and spawn tasks for units of work with the same colour.
Intel TBB is used to create and schedule tasks to take advantage of the nested task creation and work steeling (an important factor with non-homogeneous nature of the work units).

The first two categories have similar characteristics as both collision detection and continuous collision detection explore the branches of a pair of trees with early culling for pairs of branches that can be shown to have no contacts.
This, along with the potentially large variation in the number of triangles per particle, results in drastic variations in the computational expense of each particle-particle continuous or momentary comparison.
In addition to clusters being processes independently both provide an easy opportunity for parallel processing since each pairwise interaction between particles can be handled by a different thread (particle data is read-only at this stage).
Exploration of the combinations of branches can quickly become expensive for densely meshed objects so we pool this work at each depth of the tree and distribute across a proportional number of tasks.

The last category, contact resolution is harder to make parallel effectively without fundamental changes to the algorithm.
We could use locks on each of the particles to perform the updates but we observe than simple adding locks to the code with a single thread (guaranteed no-contention conditions) we see drastic decreases in performance.
While applying a significant number of additional cores may overcome this challenge the contact resolution of a single cluster is often small enough such that the challenge presented to us is how to produce enough work that
can be completed concurrently.
So any solution involving mutexs will be inefficient.
This puts an upper bound on the number of threads that should be spawned per cluster and we get our overall parallel workload from multiple clusters all spawning tasks simultaneously.
Instead of using mutexs we colour the interaction graph edges such that no particle has two connecting edges that are the same colour (see appendix?).
All edges with the same colour can then be processed concurrently.


